VariErr NLI: Separating Annotation Error from Human Label Variation

Human label variation arises when annotators assign different labels to the same item for valid reasons, while annotation errors occur when labels are assigned for invalid reasons. These two issues are prevalent in NLP benchmarks, yet existing research has studied them in isolation. To the best of our knowledge, there exists no prior work that focuses on teasing apart error from signal, especially in cases where signal is beyond black-and-white. To fill this gap, we introduce a systematic methodology and a new dataset, VariErr (variation versus error), focusing on the NLI task in English. We propose a 2-round annotation procedure with annotators explaining each label and subsequently judging the validity of label-explanation pairs. VariErr contains 7,732 validity judgments on 1,933 explanations for 500 re-annotated MNLI items. We assess the effectiveness of various automatic error detection (AED) methods and GPTs in uncovering errors versus human label variation. We find that state-of-the-art AED methods significantly underperform GPTs and humans. While GPT-4 is the best system, it still falls short of human performance. Our methodology is applicable beyond NLI, offering fertile ground for future research on error versus plausible variation, which in turn can yield better and more trustworthy NLP systems.

==> archived.tex <==
\subsection{ChaosNLI subset label probability distributions conditioned on whether the \name\ NLI label is self-validated}

The two ChaosNLI subset label probability distributions conditioned on whether the \name\ NLI label is self-corrected or not are significantly different from each other -- Welch’s t-test with \textit{equal\_var=False} gives \textit{statistic=-6.58, p-value=5.34e-10}.

\begin{figure}[h]
\centering
\includegraphics[width=0.49\textwidth]{figs/distplot_chaosnli_conditioned_self_correction.png}
\caption{ChaosNLI subset label probability distributions conditioned on whether the \name\ NLI label is self-corrected or not.}
\label{fig:distplot-chaosnli-self-correction}
\end{figure}


\subsection{ChaosNLI subset label probability distributions conditioned on the number of average valid peer judgments per explanation}


\begin{figure}[h]
\centering
\includegraphics[width=0.49\textwidth]{figs/distplot_chaosnli_conditioned_sum_per_exp.png}
\caption{ChaosNLI subset label probability distributions conditioned on the number of average valid peer-judgments per explanation.}
\label{fig:distplot-chaosnli-sum-per-exp}
\end{figure}

See Table \ref{tab:pairwise-ttest-chaosnli-distribution-sum-per-exp} for pair-wise t-test among \textit{sum-per-exp} values.
TODO: add Bonferroni correction
\begin{table}[h]
\centering
\resizebox{0.40\textwidth}{!}{
\begin{tabular}{cc|ccc}
\multicolumn{2}{c|}{sum-per-exp} 
& t-test stats & t-test p-value 
& significance\\
\hline
0 & 1 & -1.57 & 0.12 &  \\
0 & 2 & -3.79 & 0.00022 & $\ast\ast\ast$ \\
0 & 3 & -7.63 & 3.7e-12 & $\ast\ast\ast$ \\
1 & 2 & -2.76 & 0.006  & $\ast\ast$ \\
1 & 3 & -7.85 & 4.2e-14 & $\ast\ast\ast$ \\
2 & 3 & -5.71 & 1.8e-08  & $\ast\ast\ast$ \\
\end{tabular}
}
\caption{Pairwise t-test between ChaosNLI subset label probability distributions conditioned on the number of average valid peer judgments per explanation.}
\label{tab:pairwise-ttest-chaosnli-distribution-sum-per-exp}
\end{table}



\subsection{ChaosNLI distribution on self-detected error label subsets}
\begin{table}[h]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{c|ccc}
\multirow{2}{*}{\textit{self-detected error}}
& 
\multicolumn{3}{c}{ChaosNLI distributions} \\
& label & mean &  std \\
\hline
\multirow{3}{*}{Entailment}   & E & 0.5006 & 0.2367 \\
 & N & 0.3577 & 0.1667 \\
 & C & 0.1417 & 0.1941 \\
\hline
\multirow{3}{*}{Neutral}  
& E & 0.4360 & 0.2997 \\
 & N & 0.3258 & 0.1730 \\
 & C & 0.2382 & 0.2600 \\
\hline
\multirow{3}{*}{Contradiction}   
& E & 0.3429 & 0.2928 \\
& N & 0.4083 & 0.2048 \\
& C & 0.2489 & 0.2069 \\
\end{tabular}
}
\caption{Mean and standard deviation of ChaosNLI distributions on \name{} item subsets with self-detected label errors (E, N, or C).}
\label{tab:my_label}
\end{table}

\begin{figure}
\centering
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figs/barplot_chaosnli_distribution_on_peer_detected_entailment_errors.png}
\caption{Entailment Error Subset.}
\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figs/barplot_chaosnli_distribution_on_peer_detected_neutral_errors.png}
\caption{Neutral Error Subset.}
\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figs/barplot_chaosnli_distribution_on_peer_detected_contradiction_errors.png}
\caption{Contradiction Error Subset.}
\label{fig:third}
\end{subfigure}
\caption{Distribution of ChaosNLI labels on self-detected error subset items.}
\label{fig:figures}
\end{figure}


==> data_statement_v2.tex <==

\subsection{Header}

%The header should include the following:
%Dataset title
%Dataset curator(s) [name, affiliation]
%Dataset version [version, date]
%Dataset citation
%Data statement author(s) [name, affiliation]
%Data statement version [version, date]
%Data statement citation and, if available, DOI
%Links to versions of this data statement in other languages

\begin{itemize}
\item[] \textsl{Dataset Title:}
\item[] \textsl{Dataset Curator(s):}
\item[] \textsl{Dataset Version:}
\item[] \textsl{Dataset Citation:}
\item[] \textsl{Data Statement Authors:}
\item[] \textsl{Data Statement Version:}
\item[] \textsl{Data Statement Citation and DOI:}
\item[] \textsl{Links to versions of this data statement in other languages:}
\end{itemize}

\subsection{Executive Summary}

%The executive summary is a short (60–100 word) summary of the data statement that at a minimum should include: (1) a one-sentence description of the curation rationale, (2) the language(s), and (3) an overview of relevant quantitative information such as the dataset size. 

\subsection{Curation Rationale}

% The curation rationale should answer questions including: Why was this dataset created? What is the task or research question the dataset is intended to address? Which texts were included and what were the goals in selecting texts, both in the original collection and in any further sub-selection? What is the internal organization of the dataset? What constitutes a data instance?

\subsection{Documentation for Source Datasets}

% For datasets built out of pre-existing datasets, a link to a data statement for each source dataset should be included. If a data statement is not available, provide a link to a publication or other documentation. Provide links to licenses for source datasets, where applicable.

\subsection{Language Varieties}

% All of the languages and language varieties represented in the dataset should be characterized with (1) a language tag from BCP-47 identifying the language variety (e.g., en-US or yue-Hant-HK), and (2) a prose description elucidating and elaborating on the BCP-47 tag (e.g., English as spoken in Palo Alto, California; Cantonese written with traditional characters by speakers in Hong Kong who are bilingual in Mandarin).

% BCP-47: https://tools.ietf.org/rfc/bcp/bcp47.txt

\subsection{Speaker Demographic}

% All of the speaker groups represented in the dataset should be characterized with a prose description. Demographic categories are context- and culture-specific; therefore, locally appropriate categories and definitions should be used. Suggested specifications include: 

%\begin{itemize}
%\item Age
%\item Gender
%\item Race/ethnicity
%\item Socioeconomic status
%\item First language(s)
%\item Proficiency in the language(s) of the data
%\item Number of different speakers represented
%\item Presence of disordered speech
%\end{itemize}

\subsection{Annotator Demographic}

% All of the annotator groups represented in the dataset, including those who developed the guidelines, should be characterized with a prose description. Demographic categories are context- and culture-specific; therefore, locally appropriate categories and definitions should be used. Suggested specifications include:

%\begin{itemize}
%\item Age
%\item Gender
%\item Race/ethnicity
%\item Socioeconomic status
%\item First language(s)
%\item Proficiency in the language(s) of the data being annotated
%\item Number of different annotators represented
%\item Relevant training
%\end{itemize}

\subsection{Speech Situation and Text Characteristics}

% A description of the speech situation in which the linguistic production occurred and/or the relevant text characteristics should be provided. This schema element may also be used to describe the cultural context of the language practices collected. Specifications include:

%\begin{itemize}
%\item Time and place of linguistic activity
%\item Date(s) of data collection
%\item Modality (spoken, signed, written)
%\item Scripted/edited vs. spontaneous
%\item Synchronous (e.g., in-person or live online chatting) vs. asynchronous (e.g., letters, emails, forums) interaction     
%\item Speakers’ intended audience
%\item Genre (e.g., newswire vs. social media)
%\item Topic (e.g., entertainment vs. natural disaster)
%\item Non-linguistic context (e.g., photos speakers were all looking at; a game participants are playing)
%\item Additional details about the cultural context (optional)
%\end{itemize}

\subsection{Preprocessing and Data Formatting}

% A description of all preprocessing and data formatting modifications made to the data (except for annotations) should be provided, including information about any anonymization procedures. The description should also specify which, if any, tools were used to make the modifications and whether the raw data is included in the dataset.

\subsection{Capture Quality}

% A description of quality issues in data capture should be provided. This includes all types of quality issues that arise across a broad range of collection methodologies for capturing an otherwise impermanent event.

\subsection{Limitations}

% For any challenges that could not be fully addressed, a description of those challenges and characterization of the resulting limitations of the dataset should be provided.

\subsection{Metadata}

% A collection of pointers to relevant metadata should be provided. Suggestions include:

%License: Link to the license/copyright permissions for use or modification of the dataset
%Annotation Guidelines: Link to the published or online guidelines that annotators used to annotate the data
%Annotation Process: Link to documentation providing metadata about the annotation process, including protections for annotator anonymity, how annotators were compensated, and which aspects of the annotation were produced automatically
%Dataset Quality Metrics: Metrics for inter-annotator agreement and/or other numerical scores of dataset quality
%Errata: Link to the list of known errors and how to report additional ones


\begin{itemize}
\item[] \textsl{License:} 
\item[] \textsl{Annotation Guidelines:} 
\item[] \textsl{Annotation Process:} 
\item[] \textsl{Dataset Quality Metrics:} 
\item[] \textsl{Errata:}
\end{itemize}

\subsection{Disclosures and Ethical Review}

% For projects supported by funding, a description of the funding source for the dataset and relevant information (e.g., grant number) should be specified. For projects that went through an ethical approval process, a link to the institution (e.g., IRB) should be provided. In addition, include: a brief description of any consent process used; if speakers or annotators were compensated, how compensation rates were determined; any access restrictions to the data; and any potential conflicts of interest

\subsection{Other}

% Any further considerations that are relevant for the dataset should be included here. 

\subsection{Glossary}

% A list of terms and associated definitions that may be technical or unfamiliar to non-experts should be provided.

\titleformat{\subsection}[hang]{\normalfont\bfseries}{\thesection}{1em}{}

\smallskip
\subsection*{About this document}

%Include this information about the document verbatim at the end of your data statement. If you adapt the data statement template, include a note about your changes here.

A data statement is a characterization of a dataset that provides context to allow developers and users to better understand how experimental results might generalize, how software might be appropriately deployed, and what biases might be reflected in systems built on the software.

This data statement was written based on the template for the Data Statements Version 2 Schema. The template was prepared by Angelina McMillan-Major, Emily M. Bender, and Batya Friedman and can be found at \url{http://techpolicylab.uw.edu/data-statements}.

